An Efficient Black-Box Reduction from Online Learning to Multicalibration, and a New Route to $\Phi$-Regret Minimization

We give a Gordon-Greenwald-Marks (GGM) style black-box reduction from online learning to online multicalibration. Concretely, we show that to achieve high-dimensional multicalibration with respect to a class of functions $\mathcal{H}$, it suffices to combine any no-regret learner over $\mathcal {H} $ with an expected variational inequality (EVI) solver. We also prove a converse statement showing that efficient multicalibration implies efficient EVI solving, highlighting how EVIs in multicalibration mirror the role of fixed points in the GGM result for $\Phi$-regret. This first set of results addresses the high-dimensional analogue of the open question in Garg, Jung, Reingold, and Roth (SODA '24), showing that oracle-efficient online multicalibration with $\sqrt{T}$-type guarantees is possible in full generality. Furthermore, our GGM-style reduction unifies the analyses of existing algorithms, transfers guarantees from online learning to multicalibration for challenging environments with delayed observations or censored outcomes, and yields the first efficient black-box reduction between online learning and multiclass omniprediction. Our second main result is a fine-grained reduction from high-dimensional online multicalibration to (contextual) $\Phi$-regret minimization. Together with our first result, this establishes a new route from external regret to $\Phi$-regret that bypasses sophisticated fixed-point or semi-separation machinery, dramatically simplifies a result of Daskalakis, Farina, Fishelson, Pipis, and Schneider (STOC '25) while improving rates, and yields new algorithms that are robust to richer deviation classes, such as those belonging to any reproducing kernel Hilbert space.

==> algo_config.tex <==
\makeatletter
\crefname{algocf}{Algorithm}{Algorithms}
% Fix for line number alignment
%
% (From https://tex.stackexchange.com/questions/476579/how-to-align-line-numbers-horizontally-with-package-algorithm2e)
\patchcmd\algocf@Vline{\vrule}{\vrule \kern-0.4pt}{}{}
\patchcmd\algocf@Vsline{\vrule}{\vrule \kern-0.4pt}{}{}

% Algorithm2e hardcodes a right margin reduction of 1.5em.
% We revert that subtraction almost completely by appending
% to \@algocf@start an addition to \hsize.
\apptocmd{\@algocf@start}{\addtolength{\hsize}{1.4em}}{}{}

% Patch cref's \stepcounter macro to support referencing lines.
%
% (From https://tex.stackexchange.com/questions/103085/algorithm2e-cleveref-problem-with-wrong-reference-to-line-numbers)
\let\cref@old@stepcounter\stepcounter
\def\stepcounter#1{%
    \cref@old@stepcounter{#1}%
    \cref@constructprefix{#1}{\cref@result}%
    \@ifundefined{cref@#1@alias}%
    {\def\@tempa{#1}}%
    {\def\@tempa{\csname cref@#1@alias\endcsname}}%
    \protected@edef\cref@currentlabel{%
        [\@tempa][\arabic{#1}][\cref@result]%
        \csname p@#1\endcsname\csname the#1\endcsname}}

% This function makes an algorithm2e-looking ruled header for an algorithm. This is useful for creating "composite"
% algorithms split into multiple columns.
%
%
\newcounter{algocolumn@line}
\NewDocumentEnvironment {algomulticol} {O{htp!}} {%
    \begin{figure}[#1]%
        \refstepcounter{algocf}%
        \renewcommand\caption[1]{%
            \setlength{\algocf@ruledwidth}{\linewidth}%
            \@algocf@pre@ruled%
            \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
                \setlength{\algocf@lcaptionbox}{\hsize}\addtolength{\algocf@lcaptionbox}{-\AlCapHSkip}%
                \parbox[t]{\algocf@lcaptionbox}{\algocf@captiontext{\fnum@algocf}{##1}}
            }%
            \box\algocf@capbox\kern\interspacetitleruled\hrule%
            width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled%
        }%
        \setcounter{algocolumn@line}{0}
        }{%
        \@algocf@post@ruled%
    \end{figure}%
}

\NewDocumentEnvironment {algocolumn} {O{1}m+b} {%
    \scalebox{#1}{%
        \raisebox{6mm}{%
            \begin{minipage}[t]{#2}%
                \RestyleAlgo{plain}%
                \begin{algorithm}[H]%
                    \setcounter{AlgoLine}{\value{algocolumn@line}}% Continue count from previous column
                    #3%
                \end{algorithm}%
            \end{minipage}%
        }%
    }%
}{%
    \setcounter{algocolumn@line}{\value{AlgoLine}}%
}

\makeatother

% Indentation
\SetInd{0.3em}{0.6em}
\NewDocumentCommand \SmallIndentation {} {\SetInd{0.25em}{0.75em}}

% Spacing
\setlength{\interspacetitleruled}{3pt}
\newskip\algoinsideskipamount \algoinsideskipamount=2pt plus 0pt minus 0pt
\def\algoinsideskip{\vspace\algoinsideskipamount}
\SetAlgoInsideSkip{algoinsideskip}
\SetAlCapHSkip{1mm}
\setlength{\algomargin}{5mm}

% Styles
\newcommand{\fnm}[1]{\textsf{#1}}
\newcommand{\kwsty}{\normalfont\bfseries}
\newcommand{\kw}[1]{{\kwsty{}#1}}
\SetAlCapSty{kwsty}
\SetKwSty{kwsty}
\SetFuncSty{fnm}
\SetArgSty{upshape}
\SetFuncArgSty{upshape}
\SetKwComment{Hline}{}{\vspace{-3mm}\textcolor{gray}{\hrule}\vspace{1mm}}
\definecolor{darkgrey}{gray}{0.3}
\definecolor{commentcolor}{gray}{0.5}
\SetKwComment{Comment}{\color{commentcolor}[$\triangleright$\ }{}
\SetCommentSty{}
\SetNlSty{}{\color{black!50}\sffamily}{}

% Keywords
\SetKwProg{XFn}{function}{}{}
\SetKwProg{XSubr}{subroutine}{}{}
\newcommand{\Fn}[1]{\XFn{\normalfont\fnm{#1}}}
\newcommand{\Subr}[1]{\XSubr{\normalfont\fnm{#1}}}
\SetKwFor{ForEach}{for~each}{do}{end}
\crefalias{AlgoLine}{line}%
